The stratification of ISM properties in the edge-on galaxy NGC 891 revealed by NIKA2

As the millimeter wavelength range remains a largely unexplored spectral region for galaxies, the IMEGIN large program aims to map the millimeter continuum emission of 22 nearby galaxies at 1.15 and 2 mm. Using the high-resolution maps produced by the NIKA2 camera, we explore the existence of very cold dust and take possible contamination by free-free and synchrotron emission into account. We study the IR-to-radio emission coming from different regions along the galactic plane and at large vertical distances. New observations of NGC 891, using the NIKA2 camera on the IRAM 30m telescope, along with a suite of observations at other wavelengths were used to perform a multiwavelength study of the spectral energy distribution in the interstellar medium in this galaxy. This analysis was performed globally and locally, using the advanced hierarchical Bayesian fitting code, HerBIE, coupled with the THEMIS dust model. Our dust modeling is able to reproduce the near-IR to millimeter emission of NGC 891, with the exception of an excess at a level of 25% obtained by the NIKA2 observations in the outermost parts of the disk. The radio continuum and thermal dust emission are distributed differently in the disk and galaxy halo. Different dusty environments are also revealed by a multiwavelength investigation of the emission features. Our detailed decomposition at millimeter and centimeter wavelengths shows that emission at 1 mm is purely originated by dust. Radio components become progressively important with increasing wavelengths. Finally, we find that emission arising from small dust grains accounts for ~ 9.5% of the total dust mass, reaching up to 20% at large galactic latitudes. Shock waves in the outflows that shatter the dust grains might explain this higher fraction of small grains in the halo.

==> authors.tex <==
\author{S. Katsioli\inst{\ref{NOA}, \ref{UOA}}\fnmsep\thanks{\email{s.katsioli@noa.gr}}
  \and  E.~M. Xilouris  \inst{\ref{NOA}}
  \and  C. Kramer  \inst{\ref{IRAMF},\ref{IRAME}}
  \and R. Adam  \inst{\ref{LLR}}
  \and  P. Ade  \inst{\ref{Cardiff}}
  \and  H. Ajeddig  \inst{\ref{CEA}}
  \and  P. Andr\'e  \inst{\ref{CEA}}
  \and E. Artis  \inst{\ref{LPSC}}
  \and  H. Aussel  \inst{\ref{CEA}}
  \and  M. Baes  \inst{\ref{Ghent}}
  \and  A. Beelen  \inst{\ref{IAS}}
  \and  A. Beno\^it  \inst{\ref{Neel}}
  \and  S. Berta  \inst{\ref{IRAMF}}
  \and  L. Bing  \inst{\ref{LAM}}
  \and  O. Bourrion  \inst{\ref{LPSC}}
  \and  M. Calvo  \inst{\ref{Neel}}
  \and  A. Catalano  \inst{\ref{LPSC}}
  \and  C.~J.~R. Clark \inst{\ref{STSI}}
  \and  I. De~Looze  \inst{\ref{Ghent}, \ref{UCL}}
  \and  M. De~Petris  \inst{\ref{Roma}}
  \and  F.-X. D\'esert  \inst{\ref{IPAG}}
  \and  S. Doyle  \inst{\ref{Cardiff}}
  \and  E.~F.~C. Driessen  \inst{\ref{IRAMF}}
  \and  G. Ejlali  \inst{\ref{Iran}}
  \and  M. Galametz  \inst{\ref{CEA}}
  \and  F. Galliano  \inst{\ref{CEA}}
  \and  A. Gomez  \inst{\ref{CAB}}
  \and  J. Goupy  \inst{\ref{Neel}}
  \and  A. Hughes  \inst{\ref{Toulouse}}
  \and  A.~P. Jones  \inst{\ref{IAS}}
  \and  F. K\'eruzor\'e  \inst{\ref{LPSC}}
  \and  B. Ladjelate  \inst{\ref{IRAME}}
  \and  G. Lagache  \inst{\ref{LAM}}
  \and  S. Leclercq  \inst{\ref{IRAMF}}
  \and  J.-F. Lestrade  \inst{\ref{LERMA}}
  \and  J.-F. Mac\'ias-P\'erez  \inst{\ref{LPSC}}
  \and  S.~C. Madden  \inst{\ref{CEA}}
  \and  A. Maury  \inst{\ref{CEA}}
  \and  P. Mauskopf  \inst{\ref{Cardiff},\ref{Arizona}}
  \and F. Mayet  \inst{\ref{LPSC}}
  \and  A. Monfardini  \inst{\ref{Neel}}
  \and  M. Mu\~noz-Echeverr\'ia  \inst{\ref{LPSC}}
  \and  A. Nersesian  \inst{\ref{Ghent}, \ref{NOA}}
  \and  L. Pantoni  \inst{\ref{CEA}, \ref{IAS}}
  \and  D. Paradis  \inst{\ref{Toulouse}}
  \and  L. Perotto  \inst{\ref{LPSC}}
  \and  G. Pisano  \inst{\ref{Cardiff}}
  \and  N. Ponthieu  \inst{\ref{IPAG}}
  \and  V. Rev\'eret  \inst{\ref{CEA}}
  \and  A.~J. Rigby  \inst{\ref{Cardiff}}
  \and  A. Ritacco  \inst{\ref{IAS}, \ref{ENS}}
  \and  C. Romero  \inst{\ref{Pennsylvanie}}
  \and  H. Roussel  \inst{\ref{IAP}}
  \and  F. Ruppin  \inst{\ref{MIT}}
  \and  K. Schuster  \inst{\ref{IRAMF}}
  \and  S. Shu  \inst{\ref{Caltech}}
  \and  A. Sievers  \inst{\ref{IRAME}}
  \and  M.~W.~L. Smith  \inst{\ref{Cardiff}}
  \and  J. Tedros \inst{\ref{IRAME}}
  \and  F. Tabatabaei  \inst{\ref{Iran}, \ref{Laguna}}
  \and  C. Tucker  \inst{\ref{Cardiff}}
  \and  R. Zylka  \inst{\ref{IRAMF}}
}
  
  \institute{
    National Observatory of Athens, Institute for Astronomy, Astrophysics, Space Applications and Remote Sensing, Ioannou Metaxa and Vasileos Pavlou GR-15236, Athens, Greece
    \label{NOA}
    \and
    Department of Astrophysics, Astronomy \& Mechanics, Faculty of Physics, University of Athens, Panepistimiopolis, GR-15784 Zografos, Athens, Greece
    \label{UOA}
    \and
    Institut de RadioAstronomie Millim\'etrique (IRAM), Grenoble, France
    \label{IRAMF}
    \and  
    Instituto de Radioastronom\'ia Milim\'etrica (IRAM), Granada, Spain
    \label{IRAME}
    \and
    LLR (Laboratoire Leprince-Ringuet), CNRS, École Polytechnique, Institut Polytechnique de Paris, Palaiseau, France
    \label{LLR}
    \and
    School of Physics and Astronomy, Cardiff University, Queen’s Buildings, The Parade, Cardiff, CF24 3AA, UK 
    \label{Cardiff}
    \and
    Universit\'e Paris-Saclay, Universit\'e Paris Cit\'e, CEA, CNRS, AIM, 91191, Gif-sur-Yvette, France
    \label{CEA}
    \and
    Univ. Grenoble Alpes, CNRS, Grenoble INP, LPSC-IN2P3, 53, avenue des Martyrs, 38000 Grenoble, France
    \label{LPSC}
    \and
    Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA
    \label{STSI}
    \and
    Universit\'e Paris-Saclay, CNRS, Institut d'astrophysique spatiale, 91405, Orsay, France
    \label{IAS}
    \and
    Institut N\'eel, CNRS, Universit\'e Grenoble Alpes, France
    \label{Neel}
    \and
    IRAP, Université de Toulouse, CNRS, UPS, IRAP, 9 avenue colonel Roche, BP 44346, 31028 Toulouse Cedex 4, France
    \label{Toulouse}
    \and
    Aix Marseille Univ, CNRS, CNES, LAM (Laboratoire d'Astrophysique de Marseille), Marseille, France
    \label{LAM}
    \and
    Sterrenkundig Observatorium Universiteit Gent, Krijgslaan 281 S9, B-9000 Gent, Belgium
    \label{Ghent}
    \and
    Department of Physics and Astronomy, University College London, Gower Street, London WC1E 6BT, UK
    \label{UCL}
    \and 
    Dipartimento di Fisica, Sapienza Universit\`a di Roma, Piazzale Aldo Moro 5, I-00185 Roma, Italy
    \label{Roma}
    \and
    Univ. Grenoble Alpes, CNRS, IPAG, 38000 Grenoble, France 
    \label{IPAG}
    \and
    Institute for Research in Fundamental Sciences-IPM, Larak Garden,19395-5531 Tehran, Iran
    \label{Iran}
    \and
    Centro de Astrobiolog\'ia (CSIC-INTA), Torrej\'on de Ardoz, 28850 Madrid, Spain
    \label{CAB}
    \and 
    LERMA, Observatoire de Paris, PSL Research University, CNRS, Sorbonne Universit\'e, UPMC, 75014 Paris, France 
    \label{LERMA}
    \and
    School of Earth and Space Exploration and Department of Physics, Arizona State University, Tempe, AZ 85287, USA
    \label{Arizona}
    \and
    Laboratoire de Physique de l’\'Ecole Normale Sup\'erieure, ENS, PSL Research University, CNRS, Sorbonne Universit\'e, Universit\'e de Paris, 75005 Paris, France 
    \label{ENS}
    \and
    Department of Physics and Astronomy, University of Pennsylvania, 209 South 33rd Street, Philadelphia, PA, 19104, USA
    \label{Pennsylvanie}
    \and 
    Institut d'Astrophysique de Paris, Sorbonne Université, CNRS (UMR7095), 75014 Paris, France
    \label{IAP}
    \and
    Kavli Institute for Astrophysics and Space Research, Massachusetts Institute of Technology, Cambridge, MA 02139, USA
    \label{MIT}
    \and
    Caltech, Pasadena, CA 91125, USA
    \label{Caltech}
    \and
    Instituto  de  Astrofísica  de  Canarias,  Vía  L’actea  S/N,  38205  La Laguna, Spain
    \label{Laguna}
  }
